Assembling a high-precision abundance catalogue of solar twins in GALAH for phylogenetic studies

Stellar chemical abundances have proved themselves a key source of information for understanding the evolution of the Milky Way, and the scale of major stellar surveys such as GALAH have massively increased the amount of chemical data available. However, progress is hampered by the level of precision in chemical abundance data as well as the visualization methods for comparing the multidimensional outputs of chemical evolution models to stellar abundance data. Machine learning methods have greatly improved the former; while the application of tree-building or phylogenetic methods borrowed from biology are beginning to show promise with the latter. Here we analyse a sample of GALAH solar twins to address these issues. We apply The Cannon algorithm to generate a catalogue of about 40,000 solar twins with 14 high precision abundances which we use to perform a phylogenetic analysis on a selection of stars that have two different ranges of eccentricities. From our analyses we are able to find a group with mostly stars on circular orbits and some old stars with eccentric orbits whose age-[Y/Mg] relation agrees remarkably well with the chemical clocks published by previous high precision abundance studies. Our results show the power of combining survey data with machine learning and phylogenetics to reconstruct the history of the Milky Way.

==> dumptables.tex <==

\begin{table*}
    \centering
    \scalebox{1}{
        \begin{tabular}{llrrrrrr}
        \toprule
              & \textbf{min SNR} &        132(150spec) &        132(100spec) &        121(150spec) &        119(150spec) &        118(150spec) &        117(150spec) \\ \hline
        \midrule
        \textbf{Label} & \# outliers &   50 (2$\sigma$)&  7 (3$\sigma$)  &   16 (3$\sigma$) &  11 (3$\sigma$) &  6 (3$\sigma$) &  8 (3$\sigma$) \\ \hline
        teff & $\mu$ &   0.449993&  -0.885300  &   0.989125 &  -0.302386 &  -0.591440 &  -0.669211 \\ 
              & $\sigma$ &  27.833178 & 21.950394  &  30.345223 &  24.931603 &  23.002330 &  22.879008 \\ 
        logg & $\mu$ &  0.000349 & 0.003023 &  0.004237 &   0.003123 &   0.004056 &   0.003931 \\
              & $\sigma$ & 0.060557 & 0.044285 &  0.055951 &   0.053350 &   0.052613 &   0.051258 \\
        fe\_h & $\mu$ &  -0.000719 & -0.000766 &  -0.000125 &  -0.000479 &  -0.000484 &  -0.000403 \\
              & $\sigma$ & 0.023968 & 0.015250 &   0.017164 &   0.017209 &   0.016204 &   0.016413 \\
        Na\_fe & $\mu$ & -0.002201 & -0.001012 &  -0.001705 &  -0.000966 &  -0.000994 &  -0.000984 \\
              & $\sigma$ &  0.031371 & 0.019756 &   0.025572 &   0.020717 &   0.019308 &   0.018868 \\
        Mg\_fe & $\mu$ &  -0.007015 & -0.003984 &  -0.004650 &  -0.001412 &  -0.000182 &  -0.000180 \\
              & $\sigma$ & 0.046206 & 0.028590 &  0.037192 &   0.028478 &   0.029080 &   0.028366 \\
        Al\_fe & $\mu$ & -0.002653 & -0.001214 &  -0.003236 &  -0.001026 &   0.000112 &  -0.000375 \\
              & $\sigma$ & 0.048388 & 0.034202 &   0.050356 &   0.041182 &   0.039004 &   0.039579 \\
        Si\_fe & $\mu$ & 0.000020 & 0.000302 &  -0.000483 &  -0.000644 &  -0.000067 &  -0.000005 \\
              & $\sigma$ & 0.027384 & 0.015400 & 0.018998 &   0.017941 &   0.016938 &   0.016733 \\
        Ca\_fe & $\mu$ & 0.033527 & 0.002681 & 0.010688 &   0.005514 &   0.004817 &   0.005500 \\
              & $\sigma$ & 0.072921 & 0.025429 &  0.042548 &   0.030769 &   0.030356 &   0.032368 \\
        Sc\_fe & $\mu$ & -0.005396 & -0.001228 & -0.003141 &  -0.002558 &  -0.001703 &  -0.001735 \\
              & $\sigma$ & 0.030075 & 0.019716 & 0.026563 &   0.024411 &   0.024580 &   0.023851 \\
        Ti\_fe & $\mu$ &  -0.001013 & 0.000365 & -0.002057 &  -0.000933 &  -0.001275 &  -0.001417 \\
              & $\sigma$ & 0.026032 & 0.017320 &  0.022921 &   0.016780 &   0.016717 &   0.017009 \\
        Cr\_fe & $\mu$ & -0.005319 & -0.001785 &  -0.004218 &  -0.000180 &   0.000426 &   0.000258 \\
              & $\sigma$ & 0.035446 & 0.032087 &  0.044086 &   0.031169 &   0.029720 &   0.027852 \\
        Mn\_fe & $\mu$ &  0.003932 & -0.003078 &  -0.005574 &  -0.002532 &  -0.001693 &  -0.001703 \\
              & $\sigma$ & 0.052552 & 0.023533 &  0.031397 &   0.023910 &   0.024702 &   0.023760 \\
        Ni\_fe & $\mu$ & -0.010514 & 0.001456 & -0.001180 &  -0.001243 &  -0.001752 &  -0.001504 \\
              & $\sigma$ & 0.045625 & 0.030413 &  0.032211 &   0.027601 &   0.026455 &   0.025818 \\
        Cu\_fe & $\mu$ &  0.001032 & 0.000605 &  0.002990 &   0.003928 &   0.003412 &   0.003172 \\
              & $\sigma$ &  0.044358 & 0.027054 & 0.027038 &   0.028979 &   0.027399 &   0.029477 \\
        Zn\_fe & $\mu$ &  -0.004419 & -0.000284 & -0.000943 &  -0.001693 &  -0.000226 &  -0.000315 \\
              & $\sigma$ & 0.045751 & 0.031564 & 0.040461 &   0.030521 &   0.028324 &   0.027732 \\
        Y\_fe & $\mu$ &  0.006618 & 0.007391 & -0.003764 &   0.002262 &   0.003150 &   0.004571 \\
              & $\sigma$ & 0.072996 & 0.046843 &  0.073406 &   0.043910 &   0.041865 &   0.041312 \\
        Ba\_fe & $\mu$ & -0.004306 & 0.007603 &  0.004037 &   0.005080 &   0.006458 &   0.005709 \\
              & $\sigma$ & 0.077235 & 0.041975 &  0.047596 &   0.044549 &   0.043583 &   0.043068 \\
        \bottomrule
        \end{tabular}
        }
    \caption{One-to-one difference mean and standard deviations for all labels considered our The Cannon approach, for different setups of 150 training spectra.}
    \label{}
\end{table*}

\begin{table*}
    \centering
    \scalebox{1}{
        \begin{tabular}{lrrrrr}
    \toprule
    \textbf{min SNR} &        132(100spec) &        121(150spec) &        119(150spec) &        118(150spec) &        117(150spec) \\
    \textbf{Label $\sigma$} &            &            &            &            &            \\ \hline
    \midrule
teff           & -21.135867 &   9.025365 & -10.424878 & -17.356435 & -17.799512 \\
logg           & -26.871177 &  -7.606839 & -11.901661 & -13.117589 & -15.355103 \\
fe\_h           & -36.370860 & -28.385438 & -28.198173 & -32.392794 & -31.518096 \\
Na\_fe          & -37.025403 & -18.484693 & -33.961117 & -38.453950 & -39.854751 \\
Mg\_fe          & -38.124732 & -19.509396 & -38.367043 & -37.065095 & -38.610736 \\
Al\_fe          & -29.317584 &   4.067501 & -14.891216 & -19.392944 & -18.203657 \\
Si\_fe          & -43.762786 & -30.625870 & -34.485845 & -38.149263 & -38.896270 \\
Ca\_fe          & -65.127758 & -41.651646 & -57.805506 & -58.371548 & -55.612832 \\
Sc\_fe          & -34.443138 & -11.677590 & -18.832153 & -18.272919 & -20.694810 \\
Ti\_fe          & -33.464640 & -11.949284 & -35.542282 & -35.780487 & -34.659087 \\
Cr\_fe          &  -9.477371 &  24.374927 & -12.065902 & -16.155336 & -21.425476 \\
Mn\_fe          & -55.219255 & -40.254021 & -54.500914 & -52.994147 & -54.786679 \\
Ni\_fe          & -33.340955 & -29.400856 & -39.505268 & -42.017778 & -43.412659 \\
Cu\_fe          & -39.008492 & -39.045034 & -34.669165 & -38.232806 & -33.547915 \\
Zn\_fe          & -31.009920 & -11.561797 & -33.289310 & -38.090546 & -39.385297 \\
Y\_fe           & -35.828129 &   0.562596 & -39.845989 & -42.646988 & -43.405128 \\
Ba\_fe          & -45.653274 & -38.375133 & -42.319985 & -43.570745 & -44.237574 \\ \hline
\textbf{Mean}           & -36.187138 & -17.088071 & -31.800377 & -34.238904 & -34.788564 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Overall changes(in percentage) of one-to-one difference standard deviations for all labels considered our The Cannon approach, for different setups of 150 training spectra.}
    \label{tab:sigma_changes}
\end{table*}

==> phylogenetics_prev.tex <==
\section{Phylogenetic trees with GALAH solar twins} \label{sec:applications}


In this section, we are applying our validated sample of solar twins from GALAH and their higher precision abundances to the construction of phylogenetic trees. This aims at giving a step further from \cite{Jackson-21} in which we use a sample of stars observed by a spectroscopic survey and not simply taken from the literature. This has the advantage that the selection function is designed to probe stellar populations in the disk, henceforth making an interpretation of phylogenetic trees about the reconstruction of the evolution of the Galaxy more viable \citep[see][for discussion about the selection function]{Jackson-21}. The challenge here is that the precision of GALAH data is significantly lower than the abundances used in \cite{Jackson-21} because GALAH spectra and HARPS spectra have a large difference in resolution, wavelength coverage and SNR. 

%In this paper, we focus on comparing the robustness of our trees when we compute them with GALAH abundances or our new \Cannon\ ones. A full phylogenetic study of this dataset will the aim to reconstruct the history of the disk is subject to another paper. 




Here we focus on the overall support on trees made from GALAH data and made from our own \Cannon\ catalogue. A full phylogenetic study of this dataset with the aim to reconstruct the history of the disk will be subject to another paper. For our purpose,  we select solar twins from our catalogue by requesting their spectra to have SNR above 50 and the internal uncertainties in the abundances to be the highest, e.g. at least half the average uncertainty. 

From that sample we identify the star with highest eccentricity and consider it as the outgroup. Outgroups are used in phylogenetics to place roots in trees, which allows us to sort our data in an ancestral-descendant manner in the tree {\bf [Keaghan: any reference here?]}. When no evolutionary model is used as the prior -- which is the case here -- an outgroup can be used instead. This simplifies the history reconstruction and the interpretation from the tree. We attribute a star with highest eccentricity as the outgroup because its chances to have been formed from a reservoir of gas that underwent a different evolutionary history than the solar neighborhood is higher than a star with similar orbital properties to the bulk of our stars. This should make the star likely more distinct from the rest in an evolutionary sense. The outgroup star corresponds to Gaia DR3 5416434491653412480, has an eccentricity of 0.48 as reported by GALAH DR3 and corresponds to the tip number 1 in the trees.  The eccentricity distribution of the stars peaks at 0.1.  From that sample, we consider a random selection of 200 stars for the tree, which we know it has sufficient phylogenetic signal in a spiral galaxy (de Brito et al., in prep.). 




\begin{figure*}
    \hspace{-1cm}
    \includegraphics[width=0.49\textwidth]{imgs/CannonTree.png}
    \includegraphics[width=0.49\textwidth]{imgs/GalahTree.png}
    \caption{Tree of 200 stars with high precision obtained with \textit{The Cannon and GALAH}. \SB{I have downgraded the resolution of the figures so that the overleaf compiles faster.}}    \label{fig:tree1}
\end{figure*}

Trees are then calculated following \cite{Jackson-21}, namely using the classical method called Neighbor-Joining (NJ) which evaluates the hierarchical differences from an euclidean distance matrix. That distance matrix  in this case has a size of 200x200 (number of stars) and considers a selection of chemical abundance ratios which is shown to increase phylogenetic signal following the procedure of Yaxley et al (in prep). These are 91 combinations of abundance ratios obtained from 14 abundances included in our catalogue and are listed in the appendix {\bf [tbd]}. We take these combination of abundances for these 200 stars in our catalogue and in GALAH and compare the results. 

 Because the abundance ratios have associated uncertainties, we need to evaluate the support of our tree.  Following \cite{Jackson-21}, we construct NJ trees from distance matrices which are calculated taking a random value out of the normal distribution of the abundance ratio centred at its measurement with a standard deviation of its reported uncertainty. Since our abundance ratios consider a combination of abundances, we consider the uncertainty as the quadratic sum of the uncertainties of each individual abundance. This might be conservative because some abundances are known to be correlated. 


\begin{figure}
    \centering
    \includegraphics[scale=0.35]{imgs/node_support.png}
    \caption{Percentage of support in nodes}    \label{fig:node-support}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.35]{imgs/age-feh.png}
    % \includegraphics[scale=0.35]{imgs/age-feh_2.png}
        \caption{Age-metallicity relations of the stars in the clades selected from the trees of Fig.~\ref{fig:tree1}. Linear regression fits are drawn to quantify the slopes in these relations. }    \label{fig:age-met_clades}
\end{figure}


 We construct 10,000 trees by varying the abundances according to their uncertainties and study their distribution.  Figure~\ref{fig:tree1} shows the maximum clade credibility (MCC) trees. The MCC tree corresponds to one of the sampled trees which presents the largest number of nodes that are present in the rest of the sampled trees. Essentially, the tree with the highest support in all sampled trees. {\bf [Keaghan: reference for MCC?]}.   The left tree is built using \Cannon\  abundances, the right tree is built using GALAH abundances. The stars are the same, labelled in the tips with numbers from 1 to 200.  The stars are listed in ONLINE MATERIAL. 
 
In Fig.~\ref{fig:node-support} the distribution of node support is shown for the GALAH and the Cannon trees in percentage. It is the number of times a node in the MCC tree appears with respect to all nodes, therefore 1\% means that a node only appears in the MCC tree, and 100\% means that a node appears in all sampled trees.  Comparing the distributions we note that the \Cannon\ tree is overall better supported, with a larger number of nodes appearing more than 50\% of the times, while the GALAH trees are essentially all different from each other in almost every node. This result implies that the uncertainties of our \Cannon\ catalogue might allow us to build trees and perform a phylogenetic study of the Milky Way disk. 

Comparing the trees of Fig.~\ref{fig:tree1}, we see they differ, which is understandable given the distribution of the node support. If many nodes have very low support, it means there are many possible trees given our data. The differences between GALAH and \Cannon\ are of the order of the uncertainties of GALAH  hence it is expected trees will differ if built from abundances derived by \Cannon\ or reported by GALAH.  Furthermore,  the length of the tip branches differ between both trees. In fact, the GALAH ones are much larger compared to the internal branches than the \Cannon\ ones. This is an indication of poor phylogenetic signal, in the sense that the difference between two stars as reflected by the total branch length between two tips dominates over the general hierarchical structure in the tree. {\bf Keaghan, did I say that correctly? Is there a reference ?}

However, there are some similarities in the tree topologies: after few nodes from the root, there are two main clades. In the case of the \Cannon\ tree, the clades are more imbalanced than in the case of the GALAH tree. In \cite{Jackson-21} the imbalance in the tree was associated with the so-called effect of anagenesis, which reflects a gradual evolution of a single lineage through time. This is expected in the disk (see also the work of Brito-Silva et al in prep on simulated disk galaxies).  We select from  \Cannon\ tree two clades, A and B, coloured with cyan and red in the left tree of Fig.~\ref{fig:tree1}, for further study. 

The GALAH clades are more balanced, but as discussed in  Brito-Silva et al in prep, such topologies are more similar to a random tree than a phylogenetic tree in the case of galaxies, especially given the long tip branches.  In any case, we select the clades C and D, coloured with orange and magenta in the right tree of Fig.~\ref{fig:tree1}, respectively,  for being the top branches which show some level of imbalance and compare them with the stars in clade A and B. 

To check if the selected clades belong to stars that have been formed under different evolutionary environments, and thus our tree is a phylogeny, we study the age-metallicity relation. Figure~\ref{fig:age-met_clades} shows in the left panel the age-metallicity relation of the stars in the clades A, B from the \Cannon\ tree, following the color scheme of cyan and red, respectively. In the right-hand panel we show the age-metallicity relation of the stars in the clades C and D from the GALAH tree, following the color scheme of orange and magenta, respectively. The lines are the linear regression fits of the stars in each clade. 

In both cases we see that the age-metallicity relations have different slopes for the different clades. In the case of the \Cannon\ clades A and B, however, the more metal-rich sequence (B) has a steeper age-metallicity relation than the metal-poor sequence (A). This is consistent with the two sequences in age-metallicity relation discussed by \cite{nissen-2020} \citep[see also][]{jofre-2021}. We cannot directly compare the sequences with \cite{nissen-2020} because our solar twin sample {might be} biased towards older stars \citep{galah-dr3}. The fact that the more metal-rich sequence has a steeper slope is attributed to a stellar population being formed in inner parts of the galaxy, where the star formation efficiency is higher, hence the chemical enrichment more efficient. These stars have migrated to the solar neighborhood. {\bf [look at paper suggested by person in Stromlo, that chinese person, Sven?]}.  The NJ tree is therefore suggesting a shared history of these two stellar families which is consistent with previous conclusions drawn from independent studies. 

Clade C (the metal-rich stars)  from the GALAH tree has a flatter age-metallicity relation than Clade D, therefore GALAH data still does not have the precision in the abundances required to perform a robust phylogenetic study. However, GALAH data has been central for this analysis, because \Cannon\ uses the best GALAH results to perform a re-analysis which then allows us to apply phylogenetic techniques in other GALAH stars. Considering that future data releases of GALAH are expected to increase in precision,  the prospects of phylogenetic studies in GALAH are indeed very promising. 
